[Technical Report] Combining Sampling and Synopses with Worst-Case Optimal Runtime and Quality Guarantees for Graph Pattern Cardinality Estimation

Graph pattern cardinality estimation is the problem of estimating the number of embeddings of a query graph in a data graph. This fundamental problem arises, for example, during query planning in subgraph matching algorithms. There are two major approaches to solving the problem: sampling and synopsis. Synopsis (or summary)-based methods are fast and accurate if synopses capture information of graphs well. However, these methods suffer from large errors due to loss of information during summarization and inherent assumptions. Sampling-based methods are unbiased but suffer from large estimation variance due to large sample space. To address these limitations, we propose Alley, a hybrid method that combines both sampling and synopses. Alley employs 1) a novel sampling strategy, random walk with intersection, which effectively reduces the sample space, 2) branching to further reduce variance, and 3) a novel mining approach that extracts and indexes tangled patterns as synopses which are inherently difficult to estimate by sampling. By using them in the online estimation phase, we can effectively reduce the sample space while still ensuring unbiasedness. We establish that Alley has worst-case optimal runtime and approximation quality guarantees for any given error bound $\epsilon$ and required confidence $\mu$. In addition to the theoretical aspect of Alley, our extensive experiments show that Alley outperforms the state-of-the-art methods by up to orders of magnitude higher accuracy with similar efficiency.

==> dynamic.tex <==
\vspace{-0.3cm}

\section{Dynamic Ordering}\label{sec:dynamic}

This section provides an optimization technique, \emph{dynamic ordering}, to further decrease the sample space to increase the accuracy of \Alley.

In Algorithm \ref{alg:alley_sample}, the size of the local sample space, $\abs{P_{o_i}}$, is bounded to the size of the minimum set to be intersected, which is $\min_{e \in E, e \ni o_i}$ $\abs{\pi_{o_i}(F_e \,|\, p)}$. To reduce this bound, we dynamically choose $o_i$ as follows.

\vspace{-0.3cm}
%\begin{equation}\label{eq:dynamic}
\[
o_i = \left\{
\begin{array}{ll}
     \argmin_{ \substack{ u \in U } }{\min_{ \substack{e \in E \\ e \ni u} }\abs{\pi_{u}(F_e)}} & i = 1 \\
     \argmin_{ \substack{u \in U \\ \exists j < i \, \textrm{s.t.} \, (o_j, u) \in E } }{\min_{ \substack{e \in E \\ e \ni u} }\abs{\pi_{u}(F_e \,|\, p)}} & i > 1
\end{array}
\right.
\]
%\end{equation}

%\begin{equation}\label{eq:dynamic}
%o_i = \argmin_{ u \in U, \exists j < i \, \textrm{s.t.} \, (o_j, u) \in E  }{\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e \ltimes p)}}
%\end{equation}

First, we choose $o_1$, the first query vertex to sample for, as $u$ that has an incident edge $e$ whose $\pi_u(F_e)$ is the minimum among all query vertices. 
For subsequent $o_i$ $(i > 1)$, among all query vertices that are connected to an already sampled vertex, we choose the $u$ with the smallest $\min_{e \in E, e \ni u}$ $\abs{\pi_{u}(R_e \,|\, p)}$ before Line 1 in Algorithm \ref{alg:alley_sample}. The dynamic ordering tries to reduce the upper bound of each local sample space $P_{o_i}$, and thus reduces the size of the sample space, $\abs{\SampleSpace}$. We show how the dynamic ordering significantly increases the accuracy in Section \ref{sec:exp}.

In addition, dynamic ordering adds only a small amount of overhead in \Alley since we can obtain each $\abs{\pi_u(F_e \,|\, p)}$ in $O(1)$ time.
Furthermore, recall that each intersection has time complexity $O(\min_{e \in E, e \ni o_i}$ $\abs{\pi_{o_i}(R_e \,|\, p)})$ (see Section \ref{subsec:multiway}), proportional to the minimum size of $\abs{\pi_{o_i}(F_e \,|\, p)}$. 
Hence, the dynamic ordering reduces this size and often increases the efficiency of \Alley. %We also show such cases in Section \ref{sec:exp}.


%reduce the computation overhead of \Alley and further increase the accuracy. 

%While mulit-way intersection significantly increases the accuracy, it's not a free lunch. It is the main bottleneck of \Alley and limits the efficiency as in typical worst-case optimal algorithms \cite{mhedhbi2019optimizing}. %We show in Section \ref{sec:exp} that this intersection is the main bottleneck in \Alley. 
%As in such worst-case optimal algorithms, the multi-way intersection is implemented to run in $O(\min_{e \in E, e \ni o_i}$ $\abs{\pi_{o_i}(R_e \ltimes p)})$ time, proportional to the size of the minimum relation to intersect, in Line 5 of Algorithm \ref{alg:main}.
%The multi-way intersection has time complexity of $O(d(o_i) \cdot \min_{e \in E, e \ni o_i}\abs{\pi_{o_i}(R_e \ltimes p)})$ in Line 5 of Algorithm \ref{alg:main} \cite{}. Here, $d(o_i)$ is the degree of $o_i$ in $\QueryGraph$, the number of relations to intersect.
%Thus the time complexity is linear to both the number of relations to intersect, and the minimum size among this relations.
%However, it is highly likely that $e^* = \argmin_{e \in E, e \ni o_i}\abs{\pi_{o_i}(R_e \ltimes p)}$ is connected to any of precedent vertices of $o_i$, since otherwise $\abs{\pi_{o_i}(R_e \ltimes p)} = \abs{\pi_{o_i}(R_e)}$.
%In addition, the size of the local sample space for $o_i$ is bounded to $\min_{e \in E, e \ni o_i}\abs{\pi_{o_i}(R_e \ltimes p)}$ due to the intersection. %Thus $\min_{e \in E, e \ni o_i}\abs{\pi_{o_i}(R_e \ltimes p)}$ acts as an upper bound of the size of local sample space.

%Therefore, to reduce both the intersection cost and the size of local sample space, we dynamically choose $o_i$ as follows.
%\begin{equation}\label{eq:dynamic}
%o_i = \argmin_{ u \in U, u \not\in \cup_{j<i}{\{u\}} }{\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e \ltimes p)}}
%\end{equation}

%We call this dynamic ordering, and show that this idea greatly increases the accuracy and mitigate the low efficiency problem of \Alley in Section \ref{sec:exp}.

We explain how dynamic ordering works with the running example in Figure \ref{fig:alley}. %The fourth row in Figure \ref{fig:running-example}d shows two sampling orders that are dynamically determined.
First, in Line 1 of Algorithm \ref{alg:main}, we do not fix the whole $o$ but choose $o_1$ as $u_1$, since $u_1$ has an incident edge $(u_1, u_3)$ where $F_{(u_1, u_3)}$ $ = 12$ is the minimum among all $F_e$ $(e \in E)$. Then $P_{o_1} = \{v_1, v_{24}\}$ as before (Figure \ref{fig:alley}b). Assume that $v_1$ is sampled for $u_1$. Then, in the next recursive call to \SamplePotentialEmbeddings\xspace, we choose $o_2 = u_3$ since $\abs{\pi_{u_3}(F_{(u_1, u_3)} \,|\, p)} = 1$ while $\abs{\pi_{u_2}(F_{(u_1, u_2)} \,|\, p)} = 11$, $\abs{\pi_{u_2}(F_{(u_2, u_3)} \,|\, p)} = 1000$ and $\abs{\pi_{u_3}(F_{(u_2, u_3)} \,|\, p)}$ $ = 1000$. Since $P_{o_2} = P_{u_3} = \{v_2\}$ (Figure \ref{fig:alley}j and k), we sample $v_2$ for $u_3$ (Figure \ref{fig:alley}l). Finally, $o_3$ is then chosen as $u_2$, where $P_{u_2} = \{v_{13}\}$ (Figure \ref{fig:alley}m and n). Therefore, if we sample $v_1$ for $u_1$, $m_1$ can be directly sampled. The return value of each recursive call is represented in Figure \ref{fig:alley}o.
If we sample $v_{24}$ for $u_1$, $o_2 = u_2$ and $o_3 = u_3$; $m_2$ can be directly sampled through a similar process. Therefore, $\SampleSpace = \{m_1, m_2\} = \Matches$ which is the minimal possible. Each potential embedding $p \in \SampleSpace$ has probability 1/2 to be sampled, and Equation \ref{eq:variance} gives that the estimation variance is zero, achieving optimal accuracy for this example.

%$V_{o_1} = \{v_0\}$ so we sample $v_0$ for $u_0$ and append it to $p$. Then, we choose $o_2 = u_1$ since $\abs{\pi_{u_1}(R_{(u_1, u_0)} \ltimes p)} = 1$ which is the minimum. $V_{o_2} = \{v_1\}$ so we sample $v_1$ for $u_1$. Similarly, we sample $v_2$ for $o_3 = u_2$ and $v_3$ for $o_4 = u_3$. 
%Note that we used the same $o_1$ to $o_4$ in Section \ref{subsec:overview} when explaining \Alley without dynamic ordering.
%Note that $o_1$ to $o_4$ are same without dynamic ordering in Section \ref{subsec:overview}.
%However, $o_5$ is different that $o_5$ is $u_5$, not $u_4$ (overlined in Figure \ref{fig:running-example}d). This is because $\pi_{u_4}(R_{(u_4, u_0)} \ltimes p) = \{v_4, v_5, v_{16}, v_{17}, ..., v_{113}\}$, $\pi_{u_4}(R_{(u_4, u_3)} \ltimes p) = \{v_4, v_5, v_{115}, v_{116}, ..., v_{212}\}$, and $\pi_{u_4}(R_{(u_4, u_5)} \ltimes p) = \{v_4, v_5, v_6, v_7, v_9, ...\}$, while $ \pi_{u_5}(R_{(u_5, u_8)} \ltimes p)$ is only $\{v_6, v_7\}$.

%Since $V_{o_5} = \{v_6, v_7\}$, we first assume that $v_6$ is sampled for $o_5 = u_5$.
%Now we choose $o_6 = u_4$ since $\abs{\pi_{u_4}(R_{(u_4, u_5)} \ltimes p)} = 1$. After that, we choose $o_7 = u_6$, $o_8 = u_7$, $o_9 = u_8$, and $o_{10} = u_9$ (first order in the fourth row of Figure \ref{fig:running-example}d), sampling the actual embedding $m_1$ of $\QueryGraph$. The probability of sampling this $m_1$ is $\frac{1}{2}$ since $\abs{V_{o_5}} = 2$ and $\abs{V_{o_i}} = 1$ for $i \not\eq 5$.

%However, if we sample $v_7$ instead of $v_6$ for $o_5 = u_5$, the order changes to the second one in the fourth row of Figure \ref{fig:running-example}d. We choose $o_7 = u_7$ instead of $u_6$ (underlined) since $\pi_{u_7}(R_{(u_7, u_5)} \ltimes p) = \{v_{10}\}$ while $\pi_{u_6}(R_{(u_6, u_5)} \ltimes p) = \{v_{11}, v_{311}, ..., v_{409}\}$. We eventually sample $m_2$ with probability $\frac{1}{2}$, because $\abs{V_{o_5}} = 2$ and $\abs{V_{o_i}} = 1$ for $i \not\eq 5$ again.

%Without dynamic ordering, we randomly chose 
%It is clear that $\Matches = \SampleSpace$, achieving zero variance by Equation (\ref{eq:variance}) in Section \ref{subsec:samplespace}. Thus this example shows a case where dynamic ordering leads to an optimal accuracy.

\iffalse

Algorithm \ref{alg:opt} shows how we can lightly incorporate this idea in \Alley. If we na\"ively calculate (\ref{eq:dynamic}) and determine $o_i$, it will take $O(\sum_{ u \in U, u \not\in \cup_{j<i}{\{o_j\}} }d(u))$ time.
%; the first term for updating $R_e \ltimes p$ for each incident edge $e$ of $o_{i-1}$, and the second term for calculating (\ref{eq:dynamic}).
Instead, we can determine $o_i$ in $O(d(o_{i-1}))$ time. First, we maintain the order of query vertices $\{u\}$ sorted by $\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e)}$ (Line 1). This determines $o_1$. Then, for each recursive function with $i > 1$, we determine $o_i$ by comparing the $\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e \ltimes p)}$ of $u = s_c$ and for each $(o_{i-1}, u) \in E$ such that $u$ has not been sampled (Lines 6-12). Here, $c$ is the cursor for a candidate query vertex $s_c$ whose $\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e)}$ is the minimum among all unsampled query vertices. 
If $s_c$ is chosen as $o_i$, increase $c$ until we find the next unsampled query vertex in $s$ (Lines 13-16).


%The overhead of multi-way intersection. Worst-case optimal subgraph matching algorithms use intersection with cost $O(N * min R_e)$. Thus, it is linear to the minimum-size relation. However, this is likely to be $R_e \ltimes p$ with $p \cup e > 0$, so consider the minimum among $R_e \ltimes p$ such that $p \cup e > 0$.

%Rather than choosing the fixed order, dynamically order that seems to reduce the local sample space well.

%Size of local sample space is at most $R_e \ltimes p$, so we choose $min R_e \ltimes p$.

\begin{algorithm} [htb]
\caption{{\Alley}($V, E, R$)} \label{alg:opt}
\small{
    $s \leftarrow $ an order of query vertices $\{u\}$ sorted by $\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e)}$ \\
    $o \leftarrow \emptyset$ \\
    $p \leftarrow \emptyset$ \\
    $w \leftarrow \emptyset$ \\
    \Return \Recursive($V, E, R, o, s, 2, p, w, 1$) \\
    \nonl\Fn{\FMain{\Recursive($V, E, R, o, s, c, p, w, i$)}}{
        \If{$i > 1$}
        {
            $min \leftarrow \min_{e \in E, e \ni s_c}\abs{\pi_{s_c}(R_e)}$ \\
            $o_i \leftarrow s_c$ \\
            \ForEach{$(o_{i-1}, u) \in E$ s.t, $u \not\in \cup_{j<i}{\{o_j\}}$}
            {
                \If{$min > \abs{\pi_{u}(R_{(o_{i-1}, u)} \ltimes p)}$}
                {
                    $min \leftarrow \abs{\pi_{u}(R_{(o_{i-1}, u)} \ltimes p)}$ \\
                    $o_i \leftarrow u$ \\
                }
            }
            \If{$s_c = o_i$}
            {
                \Repeat{$s_c \in \cup_{j \leq i}{\{o_j\}}$}{$c \leftarrow c + 1$}%\Until
            }
        }
        Lines 5-20 in Algorithm \ref{alg:main} with additional parameters $s$ and $c$ for \Recursive
    }
}
\end{algorithm}

\fi

The dynamic ordering does not violate the probabilistic guarantees of \Alley in Section \ref{sec:proof}.
It only adds query related overhead so we can ignore it in the time complexity of \Alley as mentioned in Section \ref{subsec:agm}. %The proofs of lemmas and propositions in Section \ref{sec:proof} are not violated with the random variables we defined; we did not assume the fixed $o$ during the proofs.

Surprisingly, the idea of dynamic ordering has not been considered in existing worst-case optimal subgraph matching algorithms \cite{kankanamge2017graphflow, aref2015design, aberger2016emptyheaded, mhedhbi2019optimizing} while any of these algorithms may adopt this idea in order to reduce the intermediate results size. In detail, if we replace sampling with exhaustive search, %as in the proof of Proposition \ref{lemma:3}, 
$o$ becomes the matching order and the local sample space $P_{o_i}$ becomes the local search space for $o_i$. Therefore, the search space as well as the intermediate results size can be reduced.

==> experiment_subchapters/4.ablative_study.tex <==
\subsection{Ablative Study}\label{subsec:exp_ablative_study}

In this section we explain the effectiveness of using a hybrid approach, by combining our novel sampling strategy with TPI. 

%we change the parameters of 

==> experiment_subchapters/backup/experiment_labeled.tex <==
\vspace{-0.3cm}
\subsection{Experiments on Labeled Datasets}\label{subsec:exp_labeled}




This section presents the results on the four labeled datasets, \DBLP, \LUBM, \WatDiv, and \UniProt. %We omit the results for \DBLP due to space limitation, which are similar with other datasets. 
Table \ref{table:labeled:results} shows the q-error distribution for each dataset; "1st" and "3rd" represent the first and third quartile. Figure \ref{fig:labeled:results} shows the results for varying query topology, where we omit the results for \DBLP due to space limitation.


\noindent \underline{\textbf{Overall Results.}} For all datasets, \AlleyD achieves the best accuracy (Table \ref{table:labeled:results}). This answers Q1. Surprisingly, the average q-error of \AlleyD is only 2.04, 1.47, and 1.34 for  \DBLP, \LUBM, and \WatDiv, respectively; the estimated cardinality differs with the actual cardinality by two times on average. For the more challenging dataset \UniProt, the average q-error is larger, i.e., 48.88. However, if we remove just two queries with largest q-error, \mbox{the average q-error drops to 4.41.}

On the other hand, \CSET and \SumRDF show lower accuracy. The average q-error of \SumRDF is up to 6,800 times larger than that of \AlleyD on the \WatDiv dataset, and the average q-error of \CSET is up to 55,000 times larger on the \DBLP dataset. The gap is significantly higher for \UniProt, more than six orders of magnitude. The average q-error of \Alley is larger than \AlleyD, showing that the dynamic ordering increases the accuracy. This answers Q2. Still, \Alley is significantly more accurate than \CSET and \SumRDF. %Considering that only one query has q-error larger than 1,000, \AlleyD has stable accuracy for all datasets. The maximum q-error of \CSET and \SumRDF, however, can be up to tens of millions.
%The maximum q-error of \AlleyD is only 10.92 on the \WatDiv dataset, which shows the stable accuracy of \AlleyD. The maximum q-error of \CSET and \SumRDF, however, can be up to tens of thousands. 

\AlleyD is not only accurate but also efficient.
The average relative elapsed time of \AlleyD to the query processing time of \gStore, is only 0.53\%, 0.47\%, 0.30\%, and 0.87\% for \DBLP, \LUBM, \WatDiv, and \UniProt, respectively. Therefore, \Alley is efficient enough to be used within such exact subgraph matching systems, which we expect will lead to better query plans with negligible overheads. This answers Q3. The maximum value is only 7.08\% on the \UniProt dataset.
However, the average relative elapsed time of \SumRDF is larger than 100\% on all datasets, spending more time on the estimation than the subgraph matching. Only \SumRDF has 7 timeout queries in \UniProt while others have no such queries in any dataset. We can decrease the summary size for \SumRDF in order to decrease the computation and increase the efficiency. However, the accuracy will then fall even more due to the increased information loss. Therefore, we conclude that \SumRDF is not practical enough to use in subgraph matching systems. 


On the other hand, \CSET is significantly faster than \AlleyD on \DBLP, \LUBM, and \UniProt, due to its simple nature. Note that one can easily design a much faster estimator with sacrificing accuracy than \CSET. For \WatDiv, \CSET shows worse efficiency than \AlleyD since the number of predicates in \WatDiv is large (Table \ref{table:labeled}). The number of star-shaped structures increases exponentially, resulting in more time for selectivity estimation. % as explained in Section \ref{sec:introduction}.
Thus, \AlleyD is more efficient than \SumRDF, but less efficient than \CSET except when the number of predicates is large. However, in contrast to \SumRDF, the summary of \CSET cannot be adjusted in order to achieve better accuracy or efficiency since the summarization of \CSET is deterministic. This shows that \CSET is not practical enough.
Finally, \AlleyD shows higher efficiency than \Alley, indicating that the dynamic ordering helps not only on the accuracy but also on the efficiency. This answers Q4. In conclusion, \AlleyD is the only estimator that shows superior accuracy and reasonable efficiency on all datasets.

\noindent \underline{\textbf{Varying Query Topology.}} We plot the results for varying query topology in Figure \ref{fig:labeled:results}. The first row shows q-error distributions; the horizontal line in the middle represents the optimal q-error, 1, and separates the over- and under-estimation cases. Top, middle, and bottom crossbars represent the max, median, and min value of the distribution, where the whiskey bar represents the first and the third quartile. Here, we plot all 10 points for each query rather than just one average q-error. The second row shows the distribution of the relative estimation time to the query processing time of \gStore, and all 10 points are plotted for each query. The third row shows the average elapsed time in milliseconds. Note that \CSET and \SumRDF tend to under-estimate for all datasets and query topologies as illustrated in the running example in Section \ref{sec:introduction}.
\Alley, however, shows stable accuracy; the q-error spreads out narrowly around the horizontal line. \AlleyD further pushes the distribution close to the horizontal line. 

\CSET and \SumRDF are more accurate for linear and star queries than for snowflake and complex queries (see Figure \ref{fig:labeled:results}a). This is because their ad-hoc assumptions of the independence between predicates and the uniform probability distribution of possible world semantics, becomes even more unrealistic for more complex queries. \AlleyD, however, shows stable and high accuracy for all datasets and query topologies. 

The second and third row in Figure \ref{fig:labeled:results} shows that \SumRDF can be consistently inefficient for all query topologies. \CSET is extremely fast, while \Alley sometimes run slower than \gStore. However, \AlleyD is consistently much faster than \gStore, roughly about 100 to 1,000 times. %The third row shows the average elapsed time, presenting the scale of the estimation and the subgraph matching performances. Note that the average elapsed time of \AlleyD is always less than 100 ms.



==> experiment_subchapters/backup/experiment_samplesize.tex <==
\vspace*{-0.3cm}
\subsection{Sample Size Experiments}\label{subsec:exp_samplesize}

\begin{figure}[h!]
%\advance\leftskip-1.5cm
\centering
\includegraphics[width=0.85\columnwidth]{figures/ratio.png}
\vspace{-0.4cm}
\caption{q-error for varying sample size ratio (AIDS).}
\vspace{-0.5cm}
\label{fig:ratio}
\end{figure}

This section shows the results on our default labeled dataset, \AIDS, varying the sample size parameter of the estimators. Until now, we use 0.03 $\cdot \frac{\sum_{e \in E}{R_e}}{\abs{E}}$ as our default sample size (i.e., ratio 0.03), while here we modify the ratio from 0.0001 to 0.03 as [YS].

The accuracy of all estimators increases as the sample size increases while the efficiency decreases (Figure \ref{fig:ratio}). For all sample sizes, \Alley and \AlleyD are more accurate than \WanderJoin. Especially for ratio 0.001, the q-error of \AlleyD is less than 10 for most of the queries.
From ratio 0.003 to 0.03, the average elapsed time of \Alley and \AlleyD increases as the ratio increases. However, it is almost same from ratio 0.0001 to 0.003. This is because for such small sample sizes, the first intersection ($i = 1$ for Line 5 of Algorithm \ref{alg:main}) dominates the runtime. 
This intersection has a constant cost since $R_e$ does not change for varying sample sizes.

A user can empirically choose an adequate value of sample size, considering the trade-off between the accuracy and the efficiency. In our experiments, a user can simply choose ratio between 0.001 and 0.03 for \AlleyD; both q-error and the elasped time are reasonable where the average q-error is less than 1.25, and \AlleyD is 10 to 120 times faster than \TurboHOM.

\iffalse

\begin{figure}[h!]
\advance\leftskip-1.5cm
\includegraphics[width=1.1\columnwidth,left]{result/fig-aids-qerror-ratio.eps}
\caption{q-error for varying sample size (AIDS).}
\label{fig:ratio:acc}
\end{figure}

\begin{table}[]
\caption{Avg. q-error for varying sample size (AIDS).}
\footnotesize
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
     & 0.0001 & 0.0003 & 0.001 & 0.003 & 0.01 & 0.03 \\ \hline
    \WJ & 4,467.67 & 1,894.16 & 301.27 & 34.74 & 3.05 & 1.70 \\ \hline
    \Alley & 2,249.26 & 387.47 & 9.89 & 3.05 & 1.53 & 1.28 \\ \hline
    \AlleyD & 12.20 & 3.35 & 1.25 & 1.10 & 1.03 & 1.02 \\ \hline
\end{tabular}\label{table:ratio:acc}
\end{table}

\begin{figure}[h!]
\advance\leftskip-1.4cm
\includegraphics[width=1.1\columnwidth,left]{result/fig-aids-etime-ratio.eps}
\caption{Elapsed time for varying sample size (AIDS).}
\label{fig:ratio:time}
\end{figure}

\fi

==> experiment_subchapters/backup/experiment_scalability.tex <==
\subsection{Scalability Experiments}\label{subsec:exp_scale}

This section shows the results on the three synthetic labeled datasets, \WatDiv0.1, \WatDiv1, and \WatDiv10, with the same schema and varying sizes (Figures \ref{fig:shop:acc} and \ref{fig:shop:time}, Table \ref{table:shop:acc}). The results shows that \Alley and \AlleyD are more accurate than \WanderJoin while achieving similar efficiency, for all data size.
\textbf{Why q-error decreases as the data size increases?? Check the ratio between sample size and sample space??}
Since all three datasets have the same schema, $R_e$ for each query edge $e$ increases linearly to the data size. Thus, the sample size as well as the elapsed time of each estimator increases as the data size increases.

\begin{figure}[h!]
\advance\leftskip-1.5cm
\includegraphics[width=1.1\columnwidth,left]{result/fig-shop-qerror-bar.eps}
\caption{q-error for varying data size (WatDiv).}
\label{fig:shop:acc}
\end{figure}

\begin{table}[]
\caption{Avg. q-error for varying data size (WatDiv).}
\footnotesize
\begin{tabular}{|c||c|c|c|}
\hline
     & 0.1M & 1M & 10M \\ \hline
    \WJ & 5.58 & 1.51 & 1.13 \\ \hline
    \Alley & 1.32 & 1.08 & 1.04 \\ \hline
    \AlleyD & 1.17 & 1.02 & 1.00 \\ \hline
\end{tabular}\label{table:shop:acc}
\end{table}

\begin{figure}[h!]
\advance\leftskip-1.4cm
\includegraphics[width=1.1\columnwidth,left]{result/fig-shop-etime-bar.eps}
\caption{Elapsed time for varying data size (WatDiv).}
\label{fig:shop:time}
\end{figure}

==> experiment_subchapters/backup/experiment_unlabeled.tex <==
\vspace*{-0.3cm}
\subsection{Experiments on Unlabeled Datasets }\label{subsec:exp_unlabeled}
%\vspace*{-0.1cm}

\begin{table*}[ht]
\caption{Results on unlabeled datasets. Best value for each case is bold-faced. q-errors larger than $10^6$ are omitted.}
\advance\leftskip-0.4cm
\vspace*{-0.2cm}
\footnotesize
\setlength\tabcolsep{3pt}
\begin{tabular}{|c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
\multirow{3}{*}{Query} & \multicolumn{9}{c|}{q-error}                                                                                                                                                                                                                                       & \multicolumn{6}{c|}{Rel. elapsed time (\%)}                                                                                                                                    \\ \cline{2-16} 
                       & \multicolumn{3}{c|}{\Epinions}                                                        & \multicolumn{3}{c|}{\Amazon}                                                          & \multicolumn{3}{c|}{\Google}                                                          & \multicolumn{2}{c|}{\Epinions}                            & \multicolumn{2}{c|}{\Amazon}                              & \multicolumn{2}{c|}{\Google}                              \\ \cline{2-16} 
                       & \multicolumn{1}{c|}{\CSET} & \multicolumn{1}{c|}{\Alley} & \multicolumn{1}{c|}{\AlleyD} & \multicolumn{1}{c|}{\CSET} & \multicolumn{1}{c|}{\Alley} & \multicolumn{1}{c|}{\AlleyD} & \multicolumn{1}{c|}{\CSET} & \multicolumn{1}{c|}{\Alley} & \multicolumn{1}{c|}{\AlleyD} & \multicolumn{1}{c|}{\Alley} & \multicolumn{1}{c|}{\AlleyD} & \multicolumn{1}{c|}{\Alley} & \multicolumn{1}{c|}{\AlleyD} & \multicolumn{1}{c|}{\Alley} & \multicolumn{1}{c|}{\AlleyD} \\ \hline
$q_1$                     & 9,448                   & \textbf{1.16}              & 1.81                        & 19,536                 & 1.07                       & \textbf{1.02}               & 131,610                & 1.02                       & \textbf{1.01}               & \textbf{0.14}              & 0.16                        & \textbf{0.38}              & 0.52                        & \textbf{0.26}              & 0.27                        \\ \hline
$q_{1r}$                    & 7,354                   & 3.78                       & \textbf{1.98}               & 13,301                 & 1.05                       & \textbf{1.04}               & 67,506                 & 1.02                       & \textbf{1.01}               & \textbf{0.28}              & 0.30                        & \textbf{0.62}              & \textbf{0.62}               & \textbf{0.53}              & 0.58                        \\ \hline
$q_2$                     & 119,765                & 3.99                       & \textbf{3.08}               & 22,071                 & 1.09                       & \textbf{1.02}               & 300,286                & 1.04                       & \textbf{1.03}               & \textbf{0.00}              & \textbf{0.00}               & \textbf{0.12}              & 0.17                        & \textbf{0.08}              & 0.09                        \\ \hline
$q_{2r}$                    & 88,199                 & 4.74                       & \textbf{1.34}               & 13,617                 & \textbf{1.05}              & \textbf{1.05}               & 152,717                & 1.02                       & \textbf{1.01}               & \textbf{0.01}              & \textbf{0.01}               & \textbf{0.23}              & \textbf{0.23}               & \textbf{0.22}              & 0.23                        \\ \hline
$q_{2s}$                    & 87,776                 & 5.28                       & \textbf{1.87}               & 23,706                 & 1.05                       & \textbf{1.02}               & 245,224                & 1.04                       & \textbf{1.01}               & \textbf{0.00}              & \textbf{0.00}               & \textbf{0.12}              & 0.14                        & \textbf{0.02}              & \textbf{0.02}               \\ \hline
$q_3$                     & -                         & 2.28                       & \textbf{2.24}               & -                         & 1.06                       & \textbf{1.02}               & -                         & 1.02                       & \textbf{1.01}               & \textbf{0.02}              & \textbf{0.02}               & \textbf{0.23}              & 0.29                        & 0.10                       & \textbf{0.07}               \\ \hline
$q_{3r}$                    & -                         & \textbf{1.65}              & 2.11                        & -                         & 1.04                       & \textbf{1.03}               & -                         & \textbf{1.01}              & \textbf{1.01}               & \textbf{0.03}              & 0.04                        & 0.40                       & \textbf{0.37}               & 0.30                       & \textbf{0.26}               \\ \hline
$q_{3s}$                    & 357.0                    & 3.08                       & \textbf{1.39}               & 184.0                    & 1.05                       & \textbf{1.02}               & 4,058                  & \textbf{1.02}              & 1.03                        & \textbf{0.00}              & \textbf{0.00}               & \textbf{0.23}              & 0.28                        & \textbf{0.00}              & \textbf{0.00}               \\ \hline
$q_4$                     & -                         & 2.60                       & \textbf{1.28}               & -                         & 1.05                       & \textbf{1.02}               & -                         & \textbf{1.02}              & \textbf{1.02}               & \textbf{0.03}              & 0.04                        & \textbf{0.27}              & 0.38                        & \textbf{0.11}              & 0.15                        \\ \hline
$q_{4r}$                    & -                         & 2.06                       & \textbf{1.14}               & -                         & 1.04                       & \textbf{1.03}               & -                         & \textbf{1.01}              & \textbf{1.01}               & \textbf{0.06}              & \textbf{0.06}               & \textbf{0.44}              & 0.46                        & \textbf{0.27}              & \textbf{0.27}               \\ \hline
$q_{4s}$                    & -                         & 2.62                       & \textbf{1.16}               & -                         & 1.06                       & \textbf{1.02}               & -                         & \textbf{1.01}              & 1.03                        & \textbf{0.03}              & \textbf{0.03}               & \textbf{0.27}              & 0.37                        & \textbf{0.11}              & \textbf{0.11}               \\ \hline
$q_5$                     & -                         & 31.88                      & \textbf{1.05}               & -                         & 1.03                       & \textbf{1.00}               & -                         & \textbf{1.01}              & \textbf{1.01}               & \textbf{0.00}              & 0.03                        & \textbf{0.43}              & 1.08                        & \textbf{0.24}              & 0.45                        \\ \hline
$q_{5r}$                    & -                         & 34.86                      & \textbf{1.41}               & -                         & 1.02                       & \textbf{1.00}               & -                         & \textbf{1.01}              & \textbf{1.01}               & \textbf{0.00}              & 0.03                        & \textbf{0.80}              & 1.08                        & \textbf{0.18}              & 0.36                        \\ \hline
$q_{5s}$                    & -                         & 7.24                       & \textbf{1.20}               & -                         & 1.02                       & \textbf{1.00}               & -                         & 1.01                       & \textbf{1.00}               & \textbf{0.01}              & 0.03                        & \textbf{0.78}              & 1.04                        & \textbf{0.14}              & 0.42                        \\ \hline
\end{tabular}\label{table:unlabeled:results}
\vspace*{-0.3cm}
\end{table*}


We next discuss the results on the three unlabeled datasets, \Epinions, \Amazon, and \Google (Table \ref{table:unlabeled}). We set the timeout for \gStore at 1 hour since \gStore results in out-of-memory for some queries if ran indefinitely. We exclude the results of \SumRDF since the q-error of \SumRDF is larger than $10^6$ for all cases. We also exclude the relative elapsed time of \CSET since it is less than $0.001\%$ for all cases.

For all datasets, \Alley and \AlleyD are significantly more accurate than \CSET and \SumRDF which both suffer from huge information loss in unlabeled graphs. The minimum q-error of \CSET is 184 for $q_{3s}$ on the \Amazon dataset, while the maximum q-error of \Alley and \AlleyD is 34.88 and 3.08, respectively. As before, the dynamic ordering increases the accuracy of \Alley and often efficiency. Although \CSET is much faster than \AlleyD, the accuracy is extremely low and cannot be controlled. On the other hand, \AlleyD has the flexibility using the sample size. The experiments show that for most of the cases we can achieve superior accuracy with estimation time less than 1\% of the query processing time of \gStore. This answers Q5. Although \AlleyD is not as efficient as \CSET, it is more efficient than \SumRDF, and significantly more accurate than both \CSET and \SumRDF.

While the q-error of \AlleyD is less than 1.05 for all queries on the \Amazon and \Google datasets, it can be up to 3.08 on the \Epinions dataset. This results from the high skewness and the low number of local cycles of \Epinions, where all queries used in the experiments are cyclic.\footnote{The average clustering coefficient of \Epinions, \Amazon, and \Google, is 0.14, 0.41, and 0.51, respectively (https://snap.stanford.edu/data/), where a low clustering coefficient indicates a low number of cycles in the neighborhoods of vertices.}


==> future.tex <==
\section{Future Directions}\label{sec:future}

\subsection{Worst-case Optimal Subgraph Matching}\label{subsec:wco}

\subsection{General Join Size Estimation}\label{subsec:generaljoin}

%\subsection{Dynamic Graphs}\label{subsec:dynamicgraph}

==> revision/summary_of_revision.tex <==
\newcommand{\metareviewer}[1]{\vspace{1ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Meta-Reviewer}}}
\newcommand{\reviewcomment}[2]{\vspace{0.5ex}\noindent\underline{\textbf{Comment (#1):}} \textit{#2}\vspace{1pt}} %
\newcommand{\reviewremark}[2]{\vspace{0.5ex}\noindent\underline{\textbf{Additional Remark (#1):}} \textit{#2}\vspace{1pt}} %
\newcommand{\reviewrequiredchange}[1]{\vspace{0.5ex}\noindent\underline{\textbf{Required Change:}} \textit{#1}\vspace{1pt}} %
\newcommand{\reviewwriting}[1]{\vspace{0.5ex}\noindent\underline{\textbf{Inclusive Writing:}} \textit{#1}\vspace{1pt}} %
%\newcommand{\response}[1]{\noindent\textbf{Response:} \color{blue}#1\color{black}} %
\newcommand{\response}[1]{\noindent\textbf{Response:} #1\color{black}} %

\newcommand{\revisionhl}[1]{\textcolor{blue}{#1}}
\newcommand{\reviewer}[1]{\vspace{1ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Reviewer #1}}} %
%\newcommand{\metareviewer}[1]{\vspace{1ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Meta-Reviewer}}} %
\newcommand{\orevisions}[1]{\vspace{2ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Other Revisions}}} %

\twocolumn

\noindent {\Large \bf Response to Reviewer Comments}


\vspace{1ex}\noindent
We deeply appreciate all the reviewers' valuable comments. The comments of the reviewers were very helpful in improving the quality of the paper. In our revised version, we have carefully addressed all questions and clarification requests. We are confident that this revision reflects the reviewers’ comments and hope this revision will lead to your positive decision. For convenience, the changes to the paper are colored \revision{blue}. Our point-to-point responses to these comments are given below.


\metareviewer{}

\reviewcomment{1}{
Please see all changes requested by reviewers 1 and 2. In particular,
1) Please include a clearer discussion of the relationship between your technique and wander join in the presence of cycles.
2) Please include a more detailed discussion of the reasons for sampling by vertex with intersection rather than sampling by edge. How are they fundamentally different in effect?
3) Please discuss the impact updates would have on your approach.
4) Please clearly explain what is performed offline and what is performed online.
5) Please discuss the storage cost and running time for each phase of the combined technique.
6) Please discuss how small patterns are selected for index creation.
Optional changes) Please consider restructuring as suggested by reviewer \#2 for clarity of exposition; if you decide not to restructure, please someone make the combination of sampling and summarization the focus of the discussion.
}

\response{
We have revised the paper and addressed the concerns 1) in the responses to Comment 1 of Reviewer 1 and Additional Remark 1 of Reviewer 1, 2) in the response to Comment 2 of Reviewer 1, 3) in the response to Comment 3 of Reviewer 1, 4) in the response to Comment 2 of Reviewer 2 and Comment 3 of Reviewer 2, 5) in the responses to Comment 6 of Reviewer 2, 6) in the response to Required Change of Reviewer 2. As suggested, we have restructured the paper as in the response to Required Change of Reviewer 2.
}

%============================================================================================================REVIEWER 1
\reviewer{1}

\reviewcomment{1}{The essential principle is the same as that explored in Wander Join. The walk order, sampling failure due to a stopped walk, and other issues as mentioned in the paper have been actually already addressed in the original Wander Join work.}

\response{We have improved the explanation on these issues (Page 12, Col 1, Par 2). While sampling failures have been addressed in the Wander Join paper, nevertheless, our contribution is a new approach to carefully and effectively resolving these. The original Wander Join paper briefly mentions that too many failed random walks will slow down the convergence of estimation, and failures occur more for cyclic queries. However, resolving these is not the main contribution of the Wander Join paper. Note that finding the best walk order is not our focus.}

\textit{\textbf{In Section \ref{sec:related}}:}

\textit{\revision{... While sampling failures have been addressed in \cite{li2016wander}, it briefly mentions that too many failed random walks will slow down the convergence of estimation, and failures occur more for cyclic queries. However, resolving these is not the main contribution of \cite{li2016wander}. Instead, \cite{li2016wander} focuses on selecting a good walk order using a round-robin approach and incorporating trial and failed walks in estimation. ...}}

%Full text: The paper describes SAP HANA's optimzier extensions for m-way join enumeration. The key idea is the join unit, which encapsulates m-way joins. This is introduced as a physical operator. They provide three procedures which combines as many joins as possible into a single join unit, and only considers an m-way physical join. This reduces the search space by avoiding all possible binary join orders, and different physical plans. However, there needs to be some local optimization to decide the order of semi-joins in the m-way join, which is very much similar to binary join ordering. The details of this local optimization is unfortunately missing.
\reviewcomment{2}{Sampling vertices with intersection is an interesting variation; however, the sampling weight is still bounded to the outgoing edges of a vertex, what's the fundamental difference than sampling an edge when performing the random walk? The intuition isn't well explained.}

\response{We have improved the explanation of the two sampling strategies (Page 5, Col 2, Par 7). We have defined edge-at-a-time sampling as sampling a data edge for each query edge, vertex-at-a-time sampling as sampling a data vertex for each query vertex considering all its incident edges, and described the differences. Note that $adj_{u'}^{u}$ and $V_{u'}^{u}$ are changed notation according to Inclusive Writing of Reviewer 2.}

\textit{\textbf{In Section \ref{subsec:multiway}}:}

\textit{\revision{... We define edge-at-a-time sampling as sampling a data edge for each query edge, and vertex-at-a-time sampling as sampling a data vertex for each query vertex considering all its incident edges. To sample an embedding that matches the query, each strategy requires sampling $|E_q|$ and $|V_q|$ times, respectively. In general, $|E_q|$ is larger than $|V_q|$ (e.g., $|E_q|$ = 6, $|V_q|$ = 5 in Figure \ref{fig:running-example}a). By considering all incident edges of each query vertex, the number of candidates is smaller in vertex-at-a-time sampling, although it’s bounded to the number of outgoing edges ($|adj_{u'}^{u}|$) as in edge-at-a-time sampling except for $|P_{o_1}|$, which is bounded to $|V_{u'}^{u}|$. In Section \ref{subsec:exp_sampling_failure}, we report the number of candidates in \Alley (vertex-at-a-time) compared to \WanderJoin's (edge-at-a-time). ...}}

\textit{\textbf{In Section \ref{subsec:exp_sampling_failure}}:}

\textit{\revision{... This is due to the small sample space of \Alley, for instance, the average size of $|P_{o_i}|$ for \Alley is 107 on \LUBM ($r=0.01\%$), which is less than 0.05\% of \WJ's. ...}}

\reviewcomment{3}{What about updates?}

\response{As acknowledged in the author feedback, we have added the explanation for updates (Page 8, Col 1, Par 2). We have also added empirical results using \AIDS and \YAGO, showing that the estimation accuracy does not deteriorate much even if 5-10\% of data edges are inserted. We have reported the results in {Section \ref{subsec:exp_index_build}} in our technical paper due to the space limitation. We can further optimize performance by incrementally rebuilding the index.}

\textit{\textbf{In Section \ref{subsec:offline}}:}

\textit{\revision{... For updates, the index is built by using the RUNSTAT command, as in existing DBMSs. In order to minimize maintenance overhead, we do not update the index whenever there is an update to the graph database. When a considerable amount of updates has occurred, say 5-10\% of data edges, a DBA needs to rebuild the index by issuing RUNSTAT again. We confirmed that the estimation accuracy does not deteriorate much even if 5-10\% of data edges are inserted through experiments (see ~\cite{AAA} for the experimental results). We can further optimize performance by incrementally rebuilding the index. ...}}


\textit{\textbf{In Section \ref{subsec:exp_index_build} of \cite{AAA}}:}

\textit{\revision{... We additionally investigate the robustness of \AlleyPM regarding data updates. Edge insertion can introduce additional embeddings, which causes false negatives of the pre-built index. Therefore, \AlleyPM would increasingly underestimates as the number of inserted edges increases. In order to simulate evolving graphs, we build an index by using 90\% of data edges, and run cardinality estimation on 90\%, 92\%, 94\%, 96\%, 98\%, and 100\% of data edges. We tested with \AIDS and \YAGO. Figure 23 shows the accuracy of each amount of data edges inserted after the index build. The results show that the estimation accuracy does not deteriorate much even if 5-10\% of data edges are inserted. From the result, we can see that we do not need to rebuild a tangled pattern index until there are significant updates to the data graph. ...}}

%TODO FIGURE
\begin{figure}[h!]
\centering
\includegraphics[width=1\columnwidth]{figures/revision/Figure_23.png}
\vspace*{-0.8cm}
\end{figure}

\reviewremark{1}{please compare against the Wander Join method for join with cycles. The original Wander Join paper has detailed how to address these cases. Please also compare to the Wander Join method for walk order selection and how to deal with walk failures due to a stopped walk; see the original Wander Join paper (and its journal version) for details.}

\response{We have clarified the following in detail (Page 1, Col 2, Par 3 and Page 1, Col 2, Par 4).
The Wander Join implementation in G-CARE is based on Wander Join for cyclic graphs as in the original conference paper, where each table corresponds to a set of data edges that match a graph query edge.
The query in Figure 1a is equivalent to the join graph in Figure 1c, where the query edges ($u_{1}$, $u_{2}$), ($u_{2}$, $u_{4}$), ($u_{1}$, $u_{4}$), ($u_{1}$, $u_{3}$), ($u_{3}$, $u_{4}$), and ($u_{4}$, $u_{5}$) are converted to relations $R_{1}$, $R_{2}$, $R_{3}$, $R_{4}$, $R_{5}$, $R_{6}$, and $R_{7}$, respectively. The walk order of Wander Join is then determined on this join graph, breaking the cycles. In Figure 1c, blue edges represent this walk order. After sampling a data edge $t_{i}$ for each relation $R_{i}$, join conditions are checked between $R_{2}$, $R_{3}$, and $R_{5}$, i.e., whether the sampled vertices for $u_{4}$, $u^{\prime}_{4}$, and $u^{\prime\prime}_{4}$ are all the same. These join conditions are represented as red edges in Figure 1c.

The implementation includes techniques for walk order selection and a stopped walk; 1) generate all possible walk orders, 2) sample with different orders in a round-robin fashion, and 3) compare the variance and index lookup time to select the best order. The trial walks are also used for final estimation and stopped walks are regarded as zero-weight samples to perform an unbiased estimation.

We have additionally considered the two optimization techniques in Section 3.6 and one technique in Section 4.2.2 of the journal version. As a result, we have adopted the two optimization techniques in Section 3.6 and updated the corresponding experimental results for Wander Join in Section 8 (Page 9, Col 2, Par 2). The results show that the overall accuracy has been slightly improved, mainly due to the optimization called leaf scanning (in Section 3.6 of the journal version). At the last step of walk order, the optimization scans all qualifying edges (i.e., that complete embeddings of a query) instead of sampling just one edge. This reduces sampling failures and is especially helpful if the last step contains non-tree edges or selective predicates. We have also considered the efficiency as the original paper explains; if an adjacency list size lookup is enough to determine the sample weight, we avoid scanning all edges. As a result, the accuracy of Wander Join has improved, especially for small queries in \LUBM and \Human (Figure \ref{fig:SmallQuery}), with negligible overhead. However, for larger and complex queries in other datasets, it has less or no impact since the sampling failures are not reduced by scanning for just one step in the walk order (Figures \ref{fig:MediumQuery}, \ref{fig:LargeQuery}, and \ref{fig:TrueCard}). We suggest that pruning the candidates at every step, such as using intersections as \Alley, is essential for reducing the sampling failures in large and complex queries.

The second optimization technique in Section 3.6 of the journal version targets selective predicates, which can be translated into bound vertices (i.e., condition that a query vertex should match a specific data vertex) in graph queries. Since only \LUBM queries contain bound vertices, this optimization is effective for \LUBM only. However, the impact is negligible since the first optimization technique has already improved the performance for selective predicates.


The third optimization technique in Section 4.2.2 of the journal version guides how we should use trial walks generated in the round-robin sampling before the best order is chosen. This optimization avoids trial walks generated from walk orders with large variances, to reduce the variance of the final estimate. However, the impact is negligible or even slightly decreases the accuracy in some cases, compared to the previous version using all trial walks. We have observed that, for a large sample size and small queries, selecting a part of trial walks with small variances excludes too many sampling failures, resulting in over-estimation. Therefore, we have {decided to exclude} the third optimization technique from our experiments.


In summary, we have implemented two optimization techniques in Section 3.6 of the journal version, and the updated results for Wander Join show that the accuracy has been improved, especially for small queries.}


\textit{\textbf{In Section \ref{sec:introduction}}:}

\textit{\revision{... \WanderJoin for relational data can be translated into an estimator for graph data which performs \emph{edge-at-a-time} sampling, by regarding query edges as relations and overlapping query vertices as join keys. For example, the query graph in Figure \ref{fig:running-example}a is equivalent to a join graph in Figure \ref{fig:running-example}c. ...}}

\textit{\revision{... Blue edges in Figure \ref{fig:running-example}c represent the corresponding join path. ...}}

\textit{\revision{... If \WanderJoin starts the walk from $(v_{10}, v_{29})$ and succeeds to sample a data edge for each query edge, it finally checks the join conditions between the split query vertices \redtext{$u_4$, $u'_4$, and $u''_4$} \revision{(equivalent to red edges in Figure \ref{fig:running-example}c)}. ...}}

\textit{\textbf{In Section \ref{subsec:exp_setup}}:}

\textit{\revision{... For \WJ, we additionally implemented two optimization techniques as described in Section 3.6 of \cite{li2017wander} on top of the \GCARE implementation. ...}}

%\response{Re-numbered to Figure \ref{fig:HANA-plan}, and it is revised. And it is further explained in Section \ref{sec:challenges}.}

\reviewremark{2}{What is the essential difference between sampling edge and sampling vertex? They seem to boil down to the same from a theoretical point of view. One still needs to figure out the sampling weights (and random walk probability) based on the number of outgoing edges on a vertex.}

\response{Please refer to the response to Comment 2.}

\reviewremark{3}{The experimental results need to include a scalability experiment, as well as investigating the overhead of the proposed indexing structure in more details.}

\response{We have added a scalability experiment by using large-scale synthetic graphs and a machine with larger memory and deepened the investigation of the overhead of our indexing technique in Section 8.4 (Page 11, Col 2, Par 3 and Figure~\ref{fig:Scalability}). We generated large \LUBM datasets where the scale factor varies from 160 to 800, which is up to 10 times larger than the \LUBM dataset (with scale factor 80) we used previously. The results show that the indexing of \Alley scales well for large graphs. For investigating the indexing overhead, we have broken down the indexing time into three parts, \CalculateDomains\xspace, \GetFailureRate\xspace, and others. As expected, \CalculateDomains\xspace is the bottleneck, taking up more than 90\% of indexing time, while \GetFailureRate\xspace takes up only 3\%. We have also measured the number of calls to \CalculateDomains\xspace and \GetFailureRate\xspace\xspace. Since such numbers are similar for all data sizes, the average elapsed time of \CalculateDomains\xspace and \GetFailureRate\xspace increases linearly to the data size. In addition, \GetFailureRate\xspace is 500 times faster than \CalculateDomains\xspace on average, which indicates that our ``walk-fail-then-calculate'' approach does not add a significant overhead but effectively prunes the patterns to index.

%and the overhead of each main subroutine in Algorithm 4. As expected, CalculateDomains is the bottleneck of the indexing.

This review helped us add a new optimization technique for building indexes ((Page 8, Col 2, Par 3) in our technical paper \cite{AAA}). We have moved the description of optimization techniques of offline indexing to \cite{AAA} due to the space limitation. Before receiving the reviews, we used the same sampling ratio for both offline (index building) and online (cardinality estimation) phases, which requires rebuilding the index for different sampling ratios that will be used online. Since the sample size is proportional to sampling ratio and data size (defined in Running Environment of Section 8.1), the sample size was unnecessarily large for determining the tangled patterns in large graphs, where the sampling even became a bottleneck. Our new optimization stops sampling after the failure rate converges, i.e., using the right amount of sample size to determine tangled patterns. This increases scalability and avoids rebuilding indexes for different sampling ratios. In addition, the optimization brought a trade-off between indexing performance and online estimation accuracy. While it has investigated new tangled patterns to index and thus increased the index size, the indexing time has decreased due to less sampling overhead (Table \ref{tab:IndexPerformance}), and the new patterns have increased the online estimation accuracy (Figures \ref{fig:SmallQuery}-\ref{fig:TrueCard}, Figure \ref{fig:IndexAccuracy}, and Table \ref{tab:failure}).}


\textit{\textbf{In Section \ref{subsec:exp_setup}}:}

\textit{\revision{... For \LUBM, we use scale factor 80 by default as in \cite{park2020g}, and additionally use larger datasets with scale factors 160, 320, 480, 640, and 800; $|E_g|$ and $|V_g|$ increase linearly to the scale factor. ...}}

\textit{\revision{... We conducted experiments on a Linux machine with 16 Intel Xeon E5-2450 2.10 GHz CPUs and 32 GB RAM by default, and a machine with 512 GB RAM for scalability test, ...}}


\textit{\textbf{In Section \ref{subsec:exp_index_build}}:}

\textit{\revision{... Figure \ref{fig:Scalability} shows the indexing performance over large \LUBM datasets with scale factors from 160 to 800. The indexing time increases linearly to the scale, and \CalculateDomains\xspace dominates other functions, occupying 95\% of the total time. \GetFailureRate\xspace accounts for only 3\%. The numbers of calls for \CalculateDomains\xspace and \GetFailureRate\xspace are similar for all data sizes, which are 9K and 150K, respectively; each call to \GetFailureRate\xspace is about 500 times faster than \CalculateDomains\xspace. Therefore, our ``walk-fail-then-calculate'' approach does not incur a significant overhead yet effectively prunes the patterns to index. ...
}}

%TODO FIGURE
\begin{figure}[h!]
\centering
\includegraphics[width=0.8\columnwidth]{figures/revision/Figure_12.png}
\vspace*{-0.6cm}
\end{figure}

\textit{\textbf{In Section \ref{subsec:offline} of \cite{AAA}}:}

\textit{\revision{... Finally, instead of using a predefined sample size, we continuously update the failure rate after calculating each $w_1$ in Algorithm \ref{alg:main} and stop if the rate converges. This prevents an unnecessarily large sample size. Also, we only focus on whether $w_1$ is zero or not, so we stop each call to \SamplePotentialEmbeddings\xspace if we sample an embedding and $w_1$ is guaranteed to be nonzero. ...}}


%============================================================================================================REVIEWER 2
\reviewer{2}

\reviewcomment{1}{In their attempt to cover all comparison aspects with existing work, the authors discuss the proposed solution in a fragmented way.}

\response{We have rewritten Section \ref{sec:introduction} to discuss the limitations of existing work (synopsis and sampling-based estimators, naive combination approaches) and discussed our solution to combine sampling and synopsis in a top-down manner. We have also rewritten Sections \ref{sec:overview}-\ref{sec:index} following this structure, which discusses our overall solution in Section \ref{sec:overview} and explains each online and offline component in Section \ref{sec:sampling} and \ref{sec:index}, respectively. We have summarized the comparison aspects of competitors in Table 5 of our technical paper due to the space limitation.}


\textit{\textbf{In Section \ref{sec:introduction}}:}

\textit{\revision{... In this paper, we focus on combining two major approaches -- sampling and synopses -- to solve the graph pattern cardinality estimation problem.}
\revision{
%Sampling
Synopsis-based methods pre-build summary structures in the offline phase and use the structures to perform cardinality estimation in the online phase. Sampling-based methods perform sampling, calculate weights of samples, and aggregate these weights to estimate the cardinality in the online phase. ...}}


\textit{\revision{... Since performing a successful sampling (i.e., sampling an embedding) is important in sampling-based estimators, a naive approach to combine sampling and synopses would pre-compute embeddings by subgraph matching and use them as sample space. However, this is an NP-hard problem, and since we do not know which patterns will be queried online, we might have to calculate embeddings for all possible patterns that appear in the data graph. This is, of course, an infeasible approach. ...}}


\textit{\revision{... A second naive approach would to pre-compute \emph{domains} of small patterns (e.g., up to five edges), inspired by work for frequent pattern mining in a single large graph \cite{elseidy2014grami}. ...}}

\textit{\revision{... To address the above limitations, we present \Alley, a hybrid method that carefully combines both sampling and synopses. We first design a novel sampling strategy that reduces the sample space. Instead of using sampling only in the online phase, we interleave sampling and mining domains in the offline phase, and index only hard patterns that are inherently difficult to handle by sampling. ...}}


\textit{\revision{... Again, in the online phase, we use the domains of tangled subqueries to prune local sample spaces of queries. In short, we improve the efficiency of building synopses by combining with sampling, also the accuracy of sampling-based estimation by combining with synopses. ...}}



\textit{\textbf{In Section \ref{sec:overview}}:}

\textit{\revision{... As explained in Section \ref{sec:introduction}, a naive combination approach would mine embeddings or domains of all small-size patterns that appear in the data graph. However, this might require a tremendous amount of computation. Instead, our approach interleaves sampling during the mining to improve mining efficiency, and 
utilizes the mined domains to improve online estimation accuracy. ...}}


\textit{\textbf{In Section \ref{sec:related} of \cite{AAA}}:}

\textit{\revision{... 
Table 5 shows a summary of graph pattern cardinality estimators with four comparison aspects. The fourth aspect is based on our empirical study. ...}}

%TODO TABLE
\begin{figure}[h!]
\centering
\includegraphics[width=0.95\columnwidth]{figures/revision/Table_5.png}
\end{figure}


\reviewcomment{2}{The solution is not clearly presented as a whole (meaning the combination of sampling and creating the domains for some tangled patterns).}

\response{We have described the whole solution in Figure \ref{fig:architecture} (Page 4, Col 2), including the construction of a tangled pattern index using our sampling technique (offline phase), and estimating the cardinality of a given query using a built index (online phase). In the offline phase, the tangled pattern index is built based on the data graph $g$ only. The goal is to automatically find all tangled patterns, which are expected to result in low accuracy in the online phase.

%The patterns are investigated from smaller to larger ones, that is, each pattern is extended from its sub-patterns. A new pattern $q$ is input to our sampling-based estimator (1) along with the indexed domains of its sub-patterns (2), which are used to prune the sample space for $q$. If the ratio of sampling failures for $q$ exceeds some threshold, i.e., the pruning effect is poor, the domains of $q$ are calculated (3) and indexed as synopses. Thus, \Alley interleaves sampling with mining, that is, sampling is performed to judge the tangledness of a pattern. In the online phase, given a query graph specified by a user (4), we use the built index to prune the sample space in estimating the cardinality of the query (5).
}

\textit{\textbf{In Section \ref{sec:overview}}:}

\textit{\revision{... Figure~\ref{fig:architecture} shows the overall architecture of \Alley. 
In the offline phase, the \emph{tangled pattern index} is built based on the data graph $g$ only. The goal is to automatically find all tangled patterns, which are expected to result in low accuracy in the online phase.
The patterns are investigated from smaller to larger ones, that is, each pattern is extended from its sub-patterns. A new pattern $q$ is input to our sampling-based estimator (\textcircled{\small{1}}) along with the indexed domains of its sub-patterns (\textcircled{\small{2}}), which are used to prune the sample space for $q$. If the ratio of sampling failures for $q$ exceeds some threshold, i.e., the pruning effect is poor, the domains of $q$ are calculated (\textcircled{\small{3}}) and indexed as synopses. Thus, Alley interleaves sampling with mining, that is, sampling is performed to judge the tangledness of a pattern. In the online phase, given a query graph specified by a user (\textcircled{\small{4}}), we use the built index to prune the sample space in estimating the cardinality of the query (\textcircled{\small{5}}). ...}}


%TODO FIGURE
\begin{figure}[h!]
\centering
\includegraphics[width=0.67\columnwidth]{figures/revision/Figure_3.png}
\end{figure}

\reviewcomment{3}{There are some notions and parts of the technique that are not well-explained: what is performed online and what offline? What does this mean in practice (is a query evaluation interleaved with index construction)?}

\response{Please refer to the response to Comment 2. In the offline phase, our goal is to automatically find all tangled patterns, which are expected to result in low accuracy in the online phase. Here, since sampling is performed to judge the tangledness of a pattern, we say that sampling is interleaved with mining. In the online phase, we use the built index and sampling to estimate the cardinality of a given query.}

\reviewcomment{4}{Sometimes words and phrases are used inaccurately or colloquially: for example 'actual' embedding (there is no actual and non-actual embedding), 'terminates immediately'.}

\response{We have rephrased these and all inaccurate or colloquial terms with the help of a professional native speaker. For example, we have replaced ‘actual embedding’ with ‘embedding’ and removed ‘terminates immediately.’} %To illustrate, we have rewritten the sentence containing ‘terminates immediately’ as: if the total number of random walks exceeds s, we stop further random walks and calculate the estimate from the collected random walks so far \textcolor{red}{(Page 6, Col 1, Par 2)}.}


\textit{\textbf{In Section \ref{subsec:multiway}}:}

\textit{\revision{... For simplicity, we omit in Algorithm \ref{alg:alley_sample} that, if the total number of random walks exceeds $s$, we stop further random walks and calculate the estimate from the collected random walks so far. ...}}


\reviewcomment{5}{The 'tangled pattern index' is not defined.}

\response{We have added a formal definition of tangled pattern index in Section \ref{sec:index} (Page 6, Col 2, Par 4). }


\textit{\textbf{In Section \ref{sec:index}}:}

%TODO DEFINITION
\begin{figure}[h!]
\centering
\includegraphics[width=1\columnwidth]{figures/revision/Definition_2.png}
\end{figure}

\textit{\revision{ 
\revision{Here, if $D_q(u)$ denotes the domain of $u$ in $q$, then \emph{PointingTo} relationship from $u$ to $u^{\prime}$ represents that i) $D_{q^{\prime}}(u^{\prime}) \supseteq D_q(u)$ from the anti-monotone property (Lemma \ref{lemma:anti-monotone}) \cite{elseidy2014grami}, ii) $D_{q^{\prime}}(u^{\prime})$ is used to prune the local sample space of $u$ in $q$ (i.e., $P_{u}$) during the random walk, and iii) the rate of sampling failures of $q$ does not exceed a predefined threshold (i.e., $q$ is not tangled). If a node $n_{q}$ has no outgoing \emph{PointingTo} edge, $q$ is \emph{tangled} and the domain of each vertex in $q$ is materialized. 
%For facilitating the index lookup and preventing duplicate indexing of isomorphic patterns, we encode each pattern in a canonical form by using the BFS code~\cite{DBLP:journals/pvldb/HanLPY10}.
Figure \ref{fig:offline} shows an example index, where $q_4$ is not tangled and $q_7$ is tangled.}
 ...}}


\reviewcomment{6}{It is not clear what is the space and time complexity of some associative steps, like the computation of the intersections in sampling, and the construction and maintenance of the indexes.}

\response{We have added the space and time complexity of each step in Section \ref{sec:sampling} and \ref{sec:index}. In the case of intersections, space and time complexities are linear to the sizes of the arrays to be intersected (Page 6, Col 1, Par 2). The time complexity of each call to \SamplePotentialEmbeddings\xspace (Line \ref{Algo1:Sample} of Algorithm \ref{alg:main}) is described in (Page 6, Col 2, Par 2). We have also added the analysis of space and time complexity of indexing and searching for small queries in Section \ref{sec:index} (Page 8, Col 1, Par 3 and Page 8, Col 2, Par 1). Similar to an analysis in the original GraMi paper, we analyzed the time complexity of index construction, which is bounded by the number of all possible patterns and the complexity of Algorithm \ref{alg:offline}. Both time and space complexity decrease as $\epsilon$ decreases, where $\epsilon$ is the ratio of tangled patterns over all patterns up to $maxN$ edges.

For the maintenance of indexes, please refer to the response to Comment 3 of Reviewer 1. 
The complexity of maintenance is similar to the above, but we only calculate domains of the affected tangled patterns. Note that these are loose bounds since we do not consider 1) the impact of search space reduction by using parent tangled patterns recursively, 2) the important characteristic of tangled patterns that their domain size is much smaller than $|V_{g}|$, and 3) the optimization techniques proposed in Section \ref{subsec:offline}. For example, in \YAGO, $\epsilon$ is $10^{-5}$ and the actual average space per pattern is 4.4K whereas $|V_{g}|\times(maxN+1)$ is 76.8M.}


\textit{\textbf{In Section \ref{subsec:multiway}}:}

\textit{\revision{... Given $k$ sets of size $N_1, N_2, ..., N_k$ (sorted in ascending order), the intersection takes $O(k{N_1}\log{N_k})$ time and requires $O(N_1)$ space. ...}}

\textit{\textbf{In Section \ref{subsec:branching}}:}

\textit{\revision{... If we 1) replace Lines~\ref{alg:randomwalk_start}-\ref{alg:randomwalk_end} in Algorithm \ref{alg:alley_sample} by an exhaustive search (i.e., iterate over all $v \in P_{o_i}$ instead of sampling) and 2) replace Lines~\ref{alg:foundstart}-\ref{alg:foundend} by an exhaustive search for all $v \in P_{o_n}$ and adding $\{o_n \veryshortarrow v\}$, then \SamplePotentialEmbeddings\xspace starting from $i = 1$ becomes a specialization of \GenericJoin \cite{ngo2012worst}; each potential embedding that can be obtained at $i = n$ with $P_{o_n} \neq \emptyset$ is an embedding in $\Matches$. 
Then it is trivial that sampling without replacement makes Algorithm \ref{alg:alley_sample} a \emph{part of} a worst-case optimal algorithm, without searching for the same embedding multiple times.
In other words, sampling \emph{with} replacement cannot guarantee this; a data vertex that leads to many embeddings in the exhaustive search can be sampled multiple times, resulting in more than $O(\AGM)$ potential embeddings sampled. ...}}

\textit{\textbf{In Section \ref{subsec:offline}}:}

\textit{\revision{... Given a data graph $G=(V_{g}, E_{g}, L_{g})$, there can be $\epsilon \times|L_{g}|^{(maxN+1)}$ tangled patterns where $\epsilon$ is the ratio of tangled patterns over all patterns up to $maxN$ edges. The factor $\epsilon$ can significantly reduce time/space complexity. \CalculateDomains\xspace dominates the other functions which is bounded by $O(|E_{g}|^{maxN})$ time complexity. Therefore, the time complexity of Algorithm \ref{alg:offline} is $O(\epsilon\times|L_{g}|^{(maxN+1)}\times|E_{g}|^{maxN})$, while the space complexity is $O(\epsilon\times|L_{g}|^{(maxN+1)}\times|V_{g}|\times(maxN+1))$. The complexities of maintenance are similar to above, but we only need to calculate the domains of affected tangled patterns. Note that these are loose upper bounds since we do not consider 1) the impact of search space reduction by using pointed tangled patterns recursively, 2) the important characteristic of tangled patterns that their domain size is much smaller than $|V_{g}|$, and 3) the optimization techniques. For example, in \YAGO dataset, $\epsilon$ is $10^{-5}$ and the actual average space per pattern is 4.4K whereas $|V_{g}|\times(maxN+1)$ is 76.8M. ...}}


\textit{\textbf{In Section \ref{subsec:online}}:}

\textit{\revision{...
Given a query $q$, the number of recursive calls is $\ceil{|V_{q}|/2}$ in the worst case. For each recursive call, \PriorityFirstSearchFrom\xspace takes $O(|V_{q}|)$ time (Line~\ref{alg5:priorityfirstsearch}), and the total number of loops (Lines~\ref{alg5:greedystart}-\ref{alg5:greedyend}) is $O(2^{maxN})$. Calculating the BFS code of $\tilde{q}$ dominates \SearchDomains\xspace and takes $O(2^{|V_{\tilde{q}}|})$ where $|V_{\tilde{q}}|$ is always less than $maxN$ (Line~\ref{alg5:searchdomains}). Therefore, the time complexity of Algorithm~\ref{alg:online} is $O(|V_{q}|^2+4^{maxN}|V_{q}|)$, which is quadratic to the query size. ...}}




\reviewwriting{The paper uses proper language, although sometimes the phrasing is colloquial. There is a running example in the paper, but, frequently, the notation is so busy that it is hard to follow the examples.}

\response{We have revised the notation and examples for enhancing readability. Note that this revision has been proofread by a professional, native speaker. We have changed the notation $\pi_u(R_{(u, u’)})$ to $V_{u’}^{u}$ and $\pi_u(R_{(u, u’)} \ltimes p)$ to $adj_{u’}^{u}(v’)$ in Table \ref{table:notations}. Examples in Section~\ref{sec:sampling} were rewritten accordingly.}

\textit{\textbf{In Section \ref{subsec:notations}}:}

\textit{\revision{... We use \profwshangreen{a} set projection of $R_{(u, u')}$ onto $u'$ as $\pi_{u'}(R_{(u, u')}) := \{v' \in V_g \,|\, \exists v \in V_g: (v, v') \in R_{(u, u')}\}$ \revision{which we simplify as
$V^{u'}_{u}$, representing the set of data vertices that match $u'$ and have an incident edge in $R_{(u, u')}$.} ...}}

\textit{\revision{...
We also use $adj^{u'}_{u}(v) := \{v' \in V^{u'}_{u} \,|\, (v, v') \in E_g\}$, which is the set of adjacent vertices of $v$ in $V^{u'}_{u}$. For example, $V_{u_2}^{u_1} = \{v_1, v_2, ..., v_{10}\}$ and $adj_{u_2}^{u_1}(v_{20}) = \{v_1\}$ in Figure \ref{fig:running-example}. ...}}




\reviewrequiredchange{It would be better to restructure the paper so that the combination itself of the sampling and summarization becomes the focus of discussion. What is performed online and what offline should be also clear. For this, an appropriate running example would be nice. Then describing optimizations of the several steps of the technique can follow and strengthen the paper. The overall storage cost and efficiency of the combined technique and every step it includes should be clearly discussed. The critical part of how small patterns are selected for respective index creation should be also clear.}

\response{As explained in the response to Comment 1, we have restructured the paper and let the combination of sampling and summarization be the focus of discussion. In Section \ref{sec:introduction}, we have first explained naive combination approaches that do not use sampling during the summarization, e.g., calculating the domains for all possible patterns up to size $maxN$ without determining the tangled patterns. Then, we have explained the benefits of our combination approach, interleaving the sampling during the summarization. Since our approach indexes only tangled patterns that are advantageous for online sampling, we can greatly improve the offline indexing efficiency with a low accuracy decrease of online sampling-based estimation compared to the naive approach. This has been empirically shown in Section \ref{subsec:exp_index_build}, where the case $\zeta$ (threshold for failure rate) = 0 corresponds to the naive approach. We have explained the offline and online phase in Figure \ref{fig:architecture}. In the subsequent sections, we have used examples to help understand our ideas and analyzed the space and time complexity of each step. We have moved the description of optimization techniques of offline indexing to our technical paper \cite{AAA} due to the space limitation. We have also revised Section \ref{subsec:offline} for clarity (Page 7, Col 1, Par 2).}


\textit{\textbf{In Section \ref{subsec:offline}}:}

\textit{\revision{... Like standard frequent subgraph mining algorithms, \Alley mines from smaller to larger patterns. However, instead of mining all patterns, \Alley first performs random walks (Algorithm \ref{alg:main}) regarding each pattern as a query $q$ and the domains of sub-patterns as $D_{q_{j}}$. If the random walks fail with a high chance (above a threshold), \Alley determines that this pattern $q$ is hard to estimate its cardinality from the current index thus extends the index by mining $q$. ...}}


%============================================================================================================REVIEWER 3
\reviewer{3}

\reviewcomment{1}{It would be great if the authors could elaborate on how the proposed novel sampling/mining methods could be applied to the estimation or approximation of other graph metrics or the evaluation of graph pattern queries.}

%\response {As proposed, Figure \ref{fig:Fig_join_style} is added in introduction section.}
\response {We have added the following discussions in Section 10 (Page 12, Col 2, Par 5).}

\textit{\textbf{In Section \ref{sec:con}}:}

\textit{\revision{...
Given a pattern matching query $q$, a cost-based optimizer enumerates valid subgraph patterns of $q$ using dynamic programming and computes the cost for each pattern. The cost model calculates the cost based on the estimated cardinality. Here, \Alley computes such estimated cardinality. Furthermore, from the anti-monotone property, domains of a subquery $q'$ of $q$ can be used as the matching candidates for $q$. Since the tangled patterns have strong structural (e.g., cycles) or label correlations, the search space can be effectively reduced. ...}}

\reviewcomment{2}{The authors could shed some light on how \Alley can be effectively implemented or integrated in the state-of-the-art graph database systems. What are the possible gaps to address to have \Alley in a graph database? Also, how would \Alley benefit from a multi-core or distributed setting?}

\response{We have added the following discussions in Section 10 (Page 12, Col 2, Par 6 and Page 12, Col 2, Par 7).}

\textit{\textbf{In Section \ref{sec:con}}:}

\textit{\revision{...
While \Alley can be integrated into any in-memory graph database system in its query optimizer or for answering approximate count queries, it would be beneficial if the system has data structures optimized for intersection, which is the main bottleneck in \Alley. For example, in order to efficiently process intersections, the edges in a data graph should be stored in sorted adjacency lists. A recent graph database system, EmptyHeaded, can further benefit from its hybrid representation using bitmaps and SIMD operations, enabling faster intersections. Recent databases with GPU support might further benefit from GPU-based intersections.}}

\textit{\revision{For exploiting parallelism, index construction can be easily parallelized in a multi-core, distributed setting as in previous pattern mining studies. Our sampling-based estimation can also be easily parallelized in a multi-core setting by calling Line 6 of Algorithm 2 in parallel. However, it is non-trivial to implement an efficient online estimator in a distributed setting due to the communication overhead. Along with data partitioning and load balancing issues, we leave it as future work to extend the sampling-based estimation to a distributed setting.}}

